Non-smoothable $\mathbb{Z}/p$-actions on nuclei

In this article we construct examples of non-smoothable $\mathbb{Z}/p$-actions on indefinite spin 4-manifolds with boundary for all primes $p\geq 5$. For example, we show that for each prime $p\geq 5$ and each $n\geq 1$ there exists a locally linear $\mathbb{Z}/p$-action on the Gompf nucleus $N(2pn)$ which is not smoothable with respect to any smooth structure on $N(2pn)$. Furthermore we investigate the behavior of these actions under two different types of equivariant stabilizations with $S^{2}\times S^{2}$, namely \emph{free} and \emph{homologically trivial} stabilizations -- in particular we show that our non-smoothable $\mathbb{Z}/p$-action on $N(2pn)$ remains non-smoothable after $2n-2$ free stabilizations, and after arbitrarily many homologically trivial stabilizations. We also show that free stabilizations satisfy a Wall stabilization principle in the sense that any non-smoothable $\mathbb{Z}/p$-action becomes smoothable after some finite number free stabilizations (under certain assumptions), whereas our aforementioned result implies that homologically trivial stabilizations do not satisfy this property. The proofs of these results use equivariant $\kappa$-invariants defined by the author in \cite{Mon22}, calculations of equivariant $\eta$-invariants for the odd signature and Dirac operators on Seifert-fibered spaces, as well as an analysis of the geometric $S^{1}$-action on the Seiberg-Witten moduli spaces of Seifert-fibered spaces induced by rotation in the fibers, which may be of independent interest.

==> extra.tex <==


Let $m<n$ be positive integers. We say that \emph{$m$ is an involutive primitive root modulo $n$} if for every $a\in\ZZ_{n}^{\times}$, there exists $k\geq 0$ such that $m^{k}\equiv\pm a\pmod{n}$. In other words, $m$ is an involutive primitive root modulo $n$ if $m$ multiplicatively generates the quotient group $\ZZ_{n}^{\times}/\<-1\>$. (Note that this is a strictly weaker condition than being a \emph{primitive} root modulo $n$, as for example $2$ is an involutive primitive root but not a primitive root modulo $7$.)

For the following, let
%
\[\P:=\{p\geq 3\;|\;p\text{ is an odd prime, and }2\text{ is an involutive primitive root modulo }p.\}\]
%
For each $p\in\P$, we can construct a surjection of $\QQ$-graded additive posets
%
\[\pi':(\Q^{p},\preceq,+)\twoheadrightarrow(\QQ^{\frac{p+1}{2}},\preceq,+).\]
%

\begin{theorem}
\label{theorem:intro_kappa_2}
Let $p\in\P$ and let $(Y,\frak{s},\sigma,X,\frak{t})$ be a quintuple, where:
%
\begin{enumerate}
    \item $(Y,\frak{s},\sigma)$ is a $\ZZ_{p}$-equivariant spin rational homology sphere on which $\sigma$ acts \emph{freely},
    \item $(X,\frak{t})$ is a spin filling of $(Y,\frak{s})$ with $b_{1}(X)=0$.
\end{enumerate}
%
Furthermore, suppose that
%
\begin{enumerate}
    \item Manolescu's relative $10/8$-ths inequality is sharp for $(Y,\frak{s},X,\frak{t})$.
    \item The image of $\K(Y,\frak{s},\sigma)\subset\Q^{p}$ under the surjection $\pi':\Q^{p}\to\QQ^{\frac{p+1}{2}}$ consists of precisely one element $\vec{\kappa}=(\kappa_{0},\kappa_{1},\dots,\kappa_{\frac{p-1}{2}})\in\QQ^{\frac{p+1}{2}}$ such that $|\vec{\kappa}|=\kappa(Y,\frak{s})$.
\end{enumerate}
%
If $\sigma$ extends to a smooth, homologically trivial, pseudofree, $\frak{t}$-preserving $\ZZ_{p}$-action $\tau$ on $X$ with fixed point data $\DDD=\{(a_{i},b_{i})\}_{i=1}^{N}$, then for each $k=1,\dots,p-1$ the following formula holds:
%
\begin{align*}
    &\sum_{i=1}^{N}(-1)^{k(a_{i}+b_{i})}\csc(\tfrac{ka_{i}\pi}{p})\csc(\tfrac{kb_{i}\pi}{p}) \\
    &\qquad\qquad=4\big(\kappa(Y,\frak{s})-\kappa_{0}\big)+\tfrac{p-1}{2p}\sigma(X)-\sum_{\ell=1}^{\frac{p-1}{2}}(-1)^{k\ell}\cos(\tfrac{k\ell\pi}{p})\big(4\kappa_{\ell}+\tfrac{1}{p}\sigma(X)\big).
\end{align*}
%
\end{theorem}

\begin{remark}
It is not clear to the author whether the set $\P$ has infinite cardinality. A simple computer-assisted search shows that the only odd primes less than $100$ which are not contained in $\P$ are $17$, $41$, $43$ and $97$, and that the ratio of the number of odd primes contained in $\P$ to the number of all odd primes less than a given integer $n$ appears to converge to $\approx 67\%$ as $n$ grows large. One can show that $\P$ contains any prime of the form $p=2p'+1$ for $p'$ prime, i.e., if $p$ is the \emph{safe prime} associated to a \emph{Sophie Germain prime} $p'$. Hence an affirmative solution to the conjecture that there are infinitely many Sophie Germain primes would imply that $|\P|=\infty$. Similarly, a resolution of Artin's primitive root conjecture would also imply $|\P|=\infty$.
\end{remark}

The above proposition gives strong constraints on the possible fixed point data $\DDD$ that can arise for a smooth homologically trivial pseudofree spin $\ZZ_{p}$-action on a given manifold for $p\in\P$, which in tandem with other techniques (e.g., the $G$-Signature theorem) can help us rule out the existence of such actions.

\begin{theorem}
\label{theorem:kappa_invariants_ipr}
Let $p$ be an odd prime such that $2$ is an involutive primitive root modulo $p$, and let $(Y,\frak{s},\wh{\sigma},X,\frak{t})$ be a quintuple, where:
%
\begin{enumerate}
    \item $(Y,\frak{s},\sigma)$ is a $\ZZ_{p}$-equivariant spin rational homology sphere on which $\sigma$ acts \emph{freely},
    \item $(X,\frak{t})$ is a spin filling of $(Y,\frak{s})$ with $b_{1}(X)=0$,
\end{enumerate}
%
and suppose that Manolescu's relative $10/8$-ths inequality is sharp for $(Y,\frak{s},X,\frak{t})$, as in the statement of \ref{theorem:intro_no_smooth_extension}. Then the following statements are true:
%
\begin{enumerate}
    \item Suppose the image of $\K(Y,\frak{s},\sigma)\subset\Q^{p}$ under the surjection $\pi':\Q^{p}\to\QQ^{\frac{p+1}{2}}$ consists of at least two distinct elements $\vec{\kappa}\neq\vec{\kappa}'\in\QQ^{\frac{p+1}{2}}$, both of which are mapped to $\kappa(Y,\frak{s})$ under the surjection $\QQ^{\frac{p+1}{2}}\to\QQ$ given by $(a_{0},\dots,a_{\frac{p-1}{2}})\mapsto a_{0}+\cdots+a_{\frac{p-1}{2}}$. Then $\wh{\sigma}$ cannot extend to a smooth homologically trivial spin $\ZZ_{m}$-action over $(X,\frak{t})$.
    \item Suppose the image of $\K(Y,\frak{s},\sigma)\subset\Q^{p}$ under the surjection $\pi':\Q^{p}\to\QQ^{\frac{p+1}{2}}$ consists of precisely one element $\vec{\kappa}=(\kappa_{0},\kappa_{1},\dots,\kappa_{\frac{p-1}{2}})\in\QQ^{\frac{p+1}{2}}$ such that $\kappa_{0}+\cdots+\kappa_{\frac{p-1}{2}}=\kappa(Y,\frak{s})$, and furthermore suppose that $\wh{\sigma}$ extends to a smooth, homologically trivial, pseudofree, spin $\ZZ_{r}$-action $\wh{\tau}$ on $X$ with fixed point data $\DDD=\{(a_{i},b_{i})\}_{i=1}^{N}$. Then:
    %
    \begin{align*}
        &\sum_{i=1}^{N}S(p;0,a_{i},b_{i};(-1)^{a_{i}+b_{i}})=4(\kappa(Y,\frak{s})-\kappa_{0})+\tfrac{p-1}{2p}\sigma(X), \\
        &\sum_{i=1}^{N}S(p;\ell,a_{i},b_{i};(-1)^{\ell+a_{i}+b_{i}})=-2\kappa_{\ell}-\tfrac{1}{2p}\sigma(X)\qquad\text{ for all }\ell=1,\dots,\tfrac{p-1}{2},
    \end{align*}
    %
    where:
    %
    \[S(p;q,r,s;\varepsilon):=\tfrac{1}{p}\sum_{j=1}^{p-1}\varepsilon^{j}\cos(\tfrac{jq\pi}{p})\csc(\tfrac{jr\pi}{p})\csc(\tfrac{js\pi}{p}).\]
    %
    In particular, for each $k=1,\dots,p-1$ the following formula holds:
    %
    \begin{align*}
        &\sum_{i=1}^{N}(-1)^{k(a_{i}+b_{i})}\csc(\tfrac{ka_{i}\pi}{p})\csc(\tfrac{kb_{i}\pi}{p}) \\
        &\qquad\qquad=4\big(\kappa(Y,\frak{s})-\kappa_{0}\big)+\tfrac{p-1}{2p}\sigma(X)-\sum_{\ell=1}^{\frac{p-1}{2}}(-1)^{k\ell}\cos(\tfrac{k\ell\pi}{p})\big(4\kappa_{\ell}+\tfrac{1}{p}\sigma(X)\big).
    \end{align*}
    %
\end{enumerate}
%
\end{theorem}

For the following, let
%
\begin{align*}
&G^{\ev}_{S^{1}}:=\Pin(2)\times S^{1}, & &G^{\odd}_{S^{1}}:=\Pin(2)\times_{\ZZ_{2}} S^{1},
\end{align*}
%
where in the latter group we mod out by the diagonal $\ZZ_{2}$-subgroup $\<(-1,-1)\>\in \Pin(2)\times S^{1}$.

Now for $\frac{k}{m}\in\QQ$, let
%
\[H^{\ev}_{k,m}:=\{(e^{i\theta},e^{ik\phi/m})\;|\;0\le \theta,\phi<2\pi\}<G^{\ev}_{S^{1}},\]
%
and similarly for $\frac{2k+1}{2m}\in\QQ$ let
%
\[H^{\odd}_{2k+1,2m}:=\{(e^{i\theta},e^{i(2k+1)\psi/2m})\;|\;0\le \theta,\psi<2\pi\}<G^{\odd}_{S^{1}}.\]
%
Furthermore denote by $Z_{k,m}$ and $Z_{2k+1,2m}$ the left cosets
%
\begin{align*}
    &Z_{k,m}:=G^{\ev}_{S^{1}}/H^{\ev}_{k,m}, & &Z_{2k+1,2m}:=G^{\odd}_{S^{1}}/H^{\odd}_{2k+1,2m}.
\end{align*}
%
\begin{lemma}
%
\begin{align*}
    &III(\wt{\Sigma}Z_{k,m})=(w_{0},
\end{align*}

\end{lemma}

\section{Computing Equivariant Eta Invariants}
\label{sec:appendix}

In this section we prove Poposition \ref{prop:comparing_n_and_S} from Section \ref{sec:stabilizations}.

Let $Y=\Sigma(\alpha_{1},\dots,\alpha_{n})$ be a Seifert-fibered homology sphere, and define
%
\[\rho(Y):=\twopartdef{0}{\text{the }\alpha_{i}\text{ are all odd},}{\frac{1}{2}}{\text{one of the }\alpha_{i}\text{ is even}.}\]
%
Let $r\geq 2$ be such that $(r,\alpha_{i})=1$ for all $i=1,\dots,n$. Under this assumption, we have that $\rho_{r}:Y\to Y$ acts freely.

Let $\dirac^{\infty}$ denote the adiabatic Dirac operator from Section \ref{sec:s_1_action}. For $q\in\ZZ$ we denote by $\eta_{\dirac^{\infty}}^{(q,r)}\in\CC$ the equivariant eta-invariant of $Y$ at $(\wh{\rho}_{r})^{q}$. Using the definition of the correction term in \cite{Mon:SW} and noting that the kernel of $\dirac^{\infty}$ is zero \cite{Nic00}, we obtain:
%
\begin{equation}
n_{L}(Y,\wh{\rho}_{r},g,\nabla^{\infty})=\tfrac{1}{r}n(Y,g,\nabla^{\infty})+\tfrac{1}{2r}\sum_{q=1}^{r-1}\omega_{r}^{-qL}\eta_{\dirac^{\infty}}^{(q,r)}.
\end{equation}
%

In the upcoming article \cite{Mon:eta} we give an explicit formula for $\eta_{\dirac^{\infty}}^{(q,r)}$ in terms of the \emph{twisted Dedekind-Rademacher sum}
%
\begin{equation}
    s(b,a;x,y;p,q;r):=\sum_{j=0}^{r-1}\sum_{k=0}^{ra-1}\omega_{r}^{(j+x)p+(k+y)q}\Big(\Big(\frac{a(j+x)+b(k+y)}{ra}\Big)\Big)\Big(\Big(\frac{k+y}{ra}\Big)\Big),
\end{equation}
%
a common generalization of both the Dedekind-Rademacher sum \cite{Rademacher64} and Berndt's periodic Dedekind sum \cite{Berndt77}. Here, $\omega_{r}=e^{2\pi i/r}\in\CC$, $x\mapsto ((x))$ denotes the generalized sawtooth function
%
\[((x)):=\twopartdef{\{x\} - \frac{1}{2}}{x\not\in\ZZ,}{0}{x\in\ZZ,}\]
%
and $\{\cdot\}:\RR\to\RR$ denotes the function given by $x\mapsto x-\lfloor x\rfloor$.

For the following let $\beta_{1},\dots,\beta_{n}$ and $\gamma_{1},\dots,\gamma_{n}$ be the unique sets of integers satisfying
%
\begin{align}
    &\tfrac{\alpha\beta_{i}}{\alpha_{i}}\equiv-1\pmod{\alpha_{i}}, & &1\le \beta\le \alpha_{i}-1, \label{eq:appendix_beta} \\
    &\tfrac{\alpha\gamma_{i}}{\alpha_{i}}\equiv\rho(Y)+\sum_{i=1}^{n}\tfrac{\alpha(\alpha_{i}-1)}{2\alpha_{i}}\pmod{\alpha_{i}}, & &0\le \gamma_{i}\le \alpha_{i}-1, \label{eq:appendix_gamma}
\end{align}
%
for all $i=1,\dots, n$, where $\alpha=\alpha_{1}\cdots\alpha_{n}$.

\begin{proposition}[\cite{Mon:eta}]
\label{prop:appendix_equivariant_eta}
Let $Y=\Sigma(\alpha_{1},\dots,\alpha_{n})$ and $r\geq 2$ as above, and let $q\in\ZZ$ be such that $q\not\equiv 0\pmod{r}$. Furthermore, for each $i=1,\dots,n$ let $p_{i}\in\ZZ$ be such that $p_{i}\beta_{i}\equiv 1\pmod{\alpha_{i}}$, and let
%
\[F(x;q,r):=\threepartdef{\omega_{r}^{\{x\}q}((x))}{q\equiv 0\pmod{r},}{-\frac{i}{2}\cot(\frac{q\pi}{r})}{q\not\equiv 0\pmod{r},\;x\in\ZZ,}{-\frac{i}{2}\omega_{r}^{((x))q}\csc(\frac{q\pi}{r})}{q\not\equiv 0\pmod{r},\;x\not\in\ZZ.}\]
%
Then the following formulas hold:
%
\begin{enumerate}
    \item[(a)] If $\rho(Y)=0$, then:
    %
    \begin{align*}
        \eta_{\dirac^{\infty}}^{(q,r)}&=\sum_{i=1}^{n}\Big[2s(\beta_{i},\alpha_{i};\tfrac{\gamma_{i}}{\alpha_{i}},0;0,-q;r)+F(\{\tfrac{p_{i}\gamma_{i}}{\alpha_{i}}\};\alpha_{i}q,r)\Big] \\
        &\qquad+(\sum_{i=1}^{n}\tfrac{1}{2\alpha_{i}})i\cot(\tfrac{q\pi}{r})+\tfrac{1}{2\alpha}\csc^{2}(\tfrac{q\pi}{r}).
    \end{align*}
    %
    \item[(b)] If $\rho(Y)=\frac{1}{2}$, then:
    %
    \begin{align*}
        \eta_{\dirac^{\infty}}^{(q,r)}&=\sum_{i=1}^{n}\Big[2s(\beta_{i},\alpha_{i};\tfrac{\gamma_{i}+\frac{1}{2}\beta_{i}}{\alpha_{i}},-\tfrac{1}{2};0,-q;r)+F(\{\tfrac{p_{i}\gamma_{i}+\frac{1}{2}}{\alpha_{i}}\};\alpha_{i}q,r)\Big] \\
        &\qquad+(\sum_{i=1}^{n}\tfrac{1}{2\alpha_{i}})i\csc(\tfrac{q\pi}{r})+\tfrac{1}{2\alpha}\csc(\tfrac{q\pi}{r})\cot(\tfrac{q\pi}{r}).
    \end{align*}
    %
\end{enumerate}
%
\end{proposition}

\begin{proposition}[\cite{Mon:eta}]
\label{prop:appendix_reciprocity}
Let $b,a,p,q\in\ZZ$ be such that $b<a$, $(b,a)=1$, and let $x,y\in\RR$. Let $a_{0},\dots,a_{n}$ be defined inductively by $a_{0}=a$, $a_{1}=b$, and $a_{k}=a_{k-2}-q_{k-1}a_{k-1}$ for some $q_{1},\dots,q_{n-1}\in\ZZ_{+}$ terminating at $a_{n}=1$. Furthermore, let:
%
\begin{itemize}
    \item $x_{0},\dots,x_{n}$ be defined by $x_{0}=y$, $x_{1}=x$, and $x_{k}=x_{k-2}+q_{k-1}x_{k-1}$ for $q_{0},\dots,q_{n-1}$ as above.
    \item $p_{0},\dots,p_{n}$ be defined by $p_{0}=q$, $p_{1}=p$, and $p_{k}=p_{k-2}-q_{k-1}p_{k-1}$ for $q_{0},\dots,q_{n-1}$ as above.
\end{itemize}
%
Then for any $r\geq 2$, we have that
%
\begin{align*}
    s(b,a;x,y;p,q;r)&=(-1)^{n}F(x_{n-1}+a_{n-1}x_{n};p_{n},r)F(x_{n};p_{n-1}-a_{n-1}p_{n},r) \\
    &\qquad\qquad+\sum_{j=0}^{n-1}(-1)^{j}\scr{R}(a_{j},a_{j+1};x_{j},x_{j+1};p_{j},p_{j+1};r),
\end{align*}
%
where:
%
\begin{align*}
    &\scr{R}(b,a;x,y;p,q;r)=E(b,a;x,y;p,q;r)+F(x;q,r)F(y;p,r) \\
    &\qquad\qquad\qquad\qquad\qquad\qquad+\tfrac{b}{2a}\omega_{r}^{xq}\delta(q,r)G(y;p,r)+\tfrac{a}{2b}\omega_{r}^{yp}\delta(p,r)G(x;q,r) \\
    &\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad+\twopartdef{-\frac{1}{4}}{x,y\in\ZZ,}{0}{x\not\in\ZZ\text{ or }y\not\in\ZZ,} \\
    &E(b,a;x,y;p,q;r)=\sum_{j=0}^{r-1}\sum_{k=0}^{r-1}\omega_{r}^{(k+y)p+(j+x)q}\scr{B}_{2}\Big(\frac{b(k+y)+a(j+x)}{r}\Big), \\
    &G(x;q,r)=\twopartdef{\frac{1}{r}\omega_{r}^{xq}\Big(\{x\}^{2}-\{x\}+\frac{1}{6}\Big)}{q\equiv 0\pmod{r},}{\Big(\frac{1-2\{x\}}{2r}\Big)i\omega_{r}^{(\{x\}-\frac{1}{2})q}\csc(\frac{q\pi}{r})-\frac{1}{2r}\omega_{r}^{(\{x\}-1)q}\csc^{2}(\frac{q\pi}{r})}{q\not\equiv 0\pmod{r},} \\
    &\delta(q,r)=\twopartdef{r}{q\equiv 0\pmod{r},}{0}{\text{otherwise},} \\
    &\scr{B}_{2}(x)=\{x\}^{2}-\{x\}+\tfrac{1}{6}. \\
\end{align*}
%
\end{proposition}

The following lemma helps us calculate the sum $E(b,a;x,y;p,q;r)$:

\begin{lemma}[\cite{Mon:eta}]
The following statements are true:
%
\begin{enumerate}
    \item If $(b,r)=1$ and $b'\in\ZZ$ is such that $bb'\equiv 1\pmod{r}$, then:
    %
    \[E(b,a;x,y;p,q;r)=\delta(q-ab'p,r)\omega_{r}^{yp+xq-(ax+by)b'p}G(ax+by;b'p,r).\]
    %
    \item If $(a,r)=1$ and $a'\in\ZZ$ is such that $aa'\equiv 1\pmod{r}$, then:
    %
    \[E(b,a;x,y;p,q;r)=\delta(p-a'bq,r)\omega_{r}^{yp+xq-(ax+by)a'q}G(ax+by;a'q,r).\]
    %
\end{enumerate}
%
\end{lemma}

In the case of odd primes $p$, in \cite{Mon:eta} we prove the following periodicity property of the correction terms for the family of Brieskorn spheres $\Sigma(2,3,6n\pm 1)$:

\begin{proposition}[\cite{Mon:eta}]
\label{prop:appendix_periodicity}
Let $a\geq -7$ be such that $(a,6)=1$, let $p\geq 5$ be prime, and let $n\geq 1$ be such that $(12n+a,p)=1$. Then for any $m\geq 1$ we have that
%
\[n(\Sigma(2,3,12n+a),\wh{\rho}_{p},g,\nabla^{\infty})=n(\Sigma(2,3,12(n+mp)+a),\wh{\rho}_{p},g,\nabla^{\infty}).\]
%
\end{proposition}

In particular, the above proposition implies that
%
\begin{align*}
    &n(\Sigma(2,3,12pn-1),\wh{\rho}_{p},g,\nabla^{\infty})= n(\Sigma(2,3,12p-1),\wh{\rho}_{p},g,\nabla^{\infty}), \\
    &n(\Sigma(2,3,12pn-6p+1),\wh{\rho}_{p},g,\nabla^{\infty})=n(\Sigma(2,3,6p+1),\wh{\rho}_{p},g,\nabla^{\infty}),
\end{align*}
%
for all primes $p\geq 5$.

%-------------------------------------------------
\subsection{\texorpdfstring{Calculations for $\Sigma(2,3,12p-1)$}{Σ(2,3,12p-1)}}
\label{subsec:12p-1}

\begin{lemma}
%
\[n_{0}(\Sigma(2,3,6p+1)\]
\end{lemma}

Let $(\alpha_{1},\alpha_{2},\alpha_{3})=(2,3,12p-1)$. From (\ref{eq:appendix_beta}) and (\ref{eq:appendix_gamma}) we obtain
%
\begin{align*}
    &(\beta_{1},\beta_{2},\beta_{3})=(1,2,10p-1), & &(p_{1},p_{2},p_{3})=(1,2,12p-7), & &(\gamma_{1},\gamma_{2},\gamma_{3})=(1,0,7p-1).
\end{align*}
%
Let $q\in\ZZ$ be such that $q\not\equiv 0\pmod{p}$. By Proposition \ref{prop:appendix_equivariant_eta} we obtain
%
\begin{align*}
    \eta_{\dirac^{\infty}}^{(q,p)}&=2s(1,2;\tfrac{3}{4},-\tfrac{1}{2};0,-q;p)+2s(2,3;\tfrac{1}{6},-\tfrac{1}{2};0,-q;p) \\
    &+2s(10p-1,12p-1;\tfrac{24p-3}{24p-2},-\tfrac{1}{2};0,-q;p) \\
    &+F(\tfrac{3}{4};2q,p)+F(\tfrac{1}{6};3q,p)+F(\tfrac{12p+5}{24p-2};(12p-1)q,p) \\
    &+\tfrac{60p+1}{144p-12}i\csc(\tfrac{q\pi}{p})+\tfrac{1}{144p-12}\csc(\tfrac{q\pi}{p})\cot(\tfrac{q\pi}{p}).
\end{align*}
%
By Proposition \ref{prop:appendix_reciprocity} we have that
%
\begin{align*}
    s(1,2;\tfrac{3}{4},-\tfrac{1}{2};0,-q;p)&=-F(0;0,p)F(\tfrac{3}{4};-q,p)+\scr{R}(2,1;-\tfrac{1}{2},\tfrac{3}{4};-q,0;p) \\
    &=-F(0;0,p)F(\tfrac{3}{4};-q,p)+F(-\tfrac{1}{2};0,p)F(\tfrac{3}{4};-q,p) \\
    &\qquad\qquad+pG(\tfrac{3}{4};-q,p)+p\omega_{p}^{-3q/4}G(0;0,p).
\end{align*}
%
FINISH THIS...



%-------------------------------------------------
\subsection{\texorpdfstring{Calculations for $\Sigma(2,3,6p+1)$}{Σ(2,3,6p+1)}}
\label{subsec:6p+1}

\begin{proposition}
The following equation holds:
%
\begin{align*}
    &n_{0}(\Sigma(2,3,6p+1),\rho_{p},g,\nabla^{\infty}) \\
    &\qquad=\tfrac{1}{4p}\sum_{k=1}^{p-1}(-1)^{k}\csc(\tfrac{2k\pi}{p})\csc(\tfrac{3k\pi}{p})+\twopartdef{1}{p\equiv 1\pmod{4},}{-1}{p\equiv 3\pmod{4}.}
\end{align*}
%
\end{proposition}

Let $(\alpha_{1},\alpha_{2},\alpha_{3})=(2,3,6p+1)$. Again from (\ref{eq:appendix_beta}) and (\ref{eq:appendix_gamma}) we obtain
%
\begin{align*}
    &(\beta_{1},\beta_{2},\beta_{3})=(1,1,p), & &(p_{1},p_{2},p_{3})=(1,1,6p-5), & &(\gamma_{1},\gamma_{2},\gamma_{3})=(1,2,\tfrac{11p+1}{2}).
\end{align*}
%
By Proposition \ref{prop:appendix_equivariant_eta}, for any $q$ such that $q\not\equiv 0\pmod{p}$ we have that:
%
\begin{align*}
    \eta_{\dirac^{\infty}}^{(q,p)}&=2s(1,2;\tfrac{3}{4},-\tfrac{1}{2};0,-q;p)+2s(1,3;\tfrac{5}{6},-\tfrac{1}{2};0,-q;p) \\
    &+2s(p,6p+1;\tfrac{12p+1}{12p+2},-\tfrac{1}{2};0,-q;p) \\
    &+F(\tfrac{3}{4};2q,p)+F(\tfrac{5}{6};3q,p)+F(\tfrac{6p+7}{12p+2};(6p+1)q,p) \\
    &+\tfrac{30p+11}{72p+12}i\csc(\tfrac{q\pi}{p})+\tfrac{1}{72p+12}\csc(\tfrac{q\pi}{p})\cot(\tfrac{q\pi}{p}).
\end{align*}
%
FINISH THIS...


%-------------------------------------------------
